The Development of Energy-Recovery Linacs

Energy-recovery linacs (ERLs) have been emphasised by the recent (2020) update of the European Strategy for Particle Physics as one of the most promising technologies for the accelerator base of future high-energy physics. The current paper has been written as a base document to support and specify details of the recently published European roadmap for the development of energy-recovery linacs. The paper summarises the previous achievements on ERLs and the status of the field and its basic technology items. The main possible future contributions and applications of ERLs to particle and nuclear physics as well as industrial developments are presented. The paper includes a vision for the further future, beyond 2030, as well as a comparative data base for the main existing and forthcoming ERL facilities. A series of continuous innovations, such as on intense electron sources or high-quality superconducting cavity technology, will massively contribute to the development of accelerator physics at large. Industrial applications are potentially revolutionary and may carry the development of ERLs much further, establishing another shining example of the impact of particle physics on society and its technical foundation with a special view on sustaining nature.

==> figures/s311.tex <==
% !TeX spellcheck = en_GB

% please save images in folder images/executive

%\subsection{MESA}
%\label{subsection:MESA}
%\chapterauthor{Kurt Aulenbacher}
%---------------------------------



%\section{Overview}

 


%\label{chpt:overview}
%\sectionauthor{Your name here}

The Mainz Superconducting Energy-recovering Accelerator, MESA for short,  is going to be used for particle and nuclear physics experiments \cite{Hug:2020miu}. The superconducting RF-modules will allow CW-operation at \SI{1300}{MHz}. Two beam modes will be available.  The P2-experiment \cite{Becker:2018ggl} will use   an extracted spin-polarized beam (EB-mode) of \SI{150}{\mu A}. The MAGIX experiment  will employ windowless targets using a gas-jet technique \cite{Schlimme:2021gjx}. Because of the low areal density, the interaction of the beam with the target is minimal. Hence, energy recovery of the beam after passing the target is efficient and  higher luminosities can be achieved with a given installed RF-power.  For this "`ER-mode"', \SI{1}{mA} of beam intensity at \SI{105}{MeV} will be available in the first stage, which is planned to be increased in a second stage to \SI{10}{mA}.

 The recirculator magnet system is arranged in double sided fashion with an accelerating cryomodule of the "`ELBE"' type  on each side (see figure \ref{fig:MESA_view}). The SRF-cryomodules will operate at a gradient of \SI{12.5}{MV/m}. Four cavities of the TESLA type will then yield \SI{50}{MeV} per pass. With five \SI{180}{degree} bending arcs, this  allows  three linac passages in EB-mode and twice accelerating and twice decelerating operation in ER-mode. In ER-mode, the beam can be guided by a dedicated beamline towards the MAGIX experiment and back to the modules with the \SI{180}{degree} phase shift required for ER-operation. In EB-mode the beam is extracted after the third linac passage and guided through another external arc towards a long straight line in front of the P2-experiment. The straight will incorporate an electron beam polarimeter and 
the beam parameter stabilization for the P2-experiment.  

The injection energy is \SI{5}{MeV}, which leads to  a beam energy \SI{155}{MeV} in EB-mode and \SI{105}{MeV} in ER-mode. The fundamental power couplers and the RF-amplifiers are chosen in a way that the beam power requirement of the P2-experiment (\SI{23.25}{kW}) can be met. For ER-mode, our investigations \cite{Stoll2019} have revealed that a beam current at the experiment above \SI{10}{mA}  can be obtained as far as BBU-instability is concerned. However, a more serious limitation seems to result from the HOM-damping antennas of the TESLA-cavities. The power handling capability of the HOM antennas presently is subject to large uncertainties. Their thermal conductivity has been improved for the MESA cavities \cite{Stengler:2020vrh}. Therefore, the  limitation for the beam current at the experiment is presently believed to be within the range of the design value of \SI{1}{mA}. Further improvements, for instance by coating of the antennas with material of higher $T_C$ are presently under investigation. The MAGIX experiment will operate with a windowless gas jet target. Together with the \SI{1}{mA} MESA beam, luminosities of \SI{>1E35}{cm^{-2}s^{-1}}  are possible. This luminosity can be run permanently  while complying with radiation production regulations valid for our institution, at least for targets with low nuclear charge like hydrogen or helium \cite{Ledroit:2021stt}. 
 


%--------------------------------- 
 
\begin{figure}[htbp]
 \centering
 \includegraphics[width=1.0\textwidth]{figures/MESA_view.png}
 \caption{Overview of MESA accelerator components. Blue, yellow and red indicators stand for dipoles, quadrupoles and beam position monitors, respectively.}
 \label{fig:MESA_view}
\end{figure}




==> s47.tex <==
\section{Power to ERLs} \label{sec:key_challenges:power}
% description of available systems and forthcoming innovation (FRT eg) 
Erk Jensen, Nick Shipman


Power sources (klystrons, IOTs, SSPAs). Power couplers. 

In normal operation, steady state CW RF power is almost zero if beam energy is fully recovered. The power needed will be given by the need to keep the fields in the cavities in the presence of both, accelerated and decelerated beams and in the presence of microphonics. This is where the FRT comes in since it can reduce the effect of microphonics. 

For Nick to describe the FRT and its beauty.

\begin{equation}\label{eqn:Pf}
P_{RF} = \frac{V_c^2}{4{}^R{\mskip -5mu/\mskip -3mu}_QQ_L}\frac{\beta+1}{\beta}\bigg[ 1+\bigg(2Q_L\frac{\Delta\omega_{\mu}}{\omega_0}\bigg)^2\bigg]
\end{equation}

Assuming you have microphonics completely suppressed, power needs will be dominated by transients, both when filling and emptying the machine or if the beam suddenly vanishes due to a problem. The RF system must be dimensioned for this case, so we have to study failure modes. Nonetheless, in normal operation the average power consumption can be very low.

The situation is very different for the injector cryomodule(s), where real power has to be fed through the cavities to the beam (example: \SI{5}{mA}$\times$ \SI{6}{MV} = \SI{30}{kW} CW!


==> s48.tex <==
\section{Cryogenics}
Patxi Duthil, 

